Higher degree sum-of-squares relaxations robust against oblivious outliers

We consider estimation models of the form $Y=X^*+N$, where $X^*$ is some $m$-dimensional signal we wish to recover, and $N$ is symmetrically distributed noise that may be unbounded in all but a small $\alpha$ fraction of the entries. We introduce a family of algorithms that under mild assumptions recover the signal $X^*$ in all estimation problems for which there exists a sum-of-squares algorithm that succeeds in recovering the signal $X^*$ when the noise $N$ is Gaussian. This essentially shows that it is enough to design a sum-of-squares algorithm for an estimation problem with Gaussian noise in order to get the algorithm that works with the symmetric noise model. Our framework extends far beyond previous results on symmetric noise models and is even robust to adversarial perturbations. As concrete examples, we investigate two problems for which no efficient algorithms were known to work for heavy-tailed noise: tensor PCA and sparse PCA. For the former, our algorithm recovers the principal component in polynomial time when the signal-to-noise ratio is at least $\tilde{O}(n^{p/4}/\alpha)$, that matches (up to logarithmic factors) current best known algorithmic guarantees for Gaussian noise. For the latter, our algorithm runs in quasipolynomial time and matches the state-of-the-art guarantees for quasipolynomial time algorithms in the case of Gaussian noise. Using a reduction from the planted clique problem, we provide evidence that the quasipolynomial time is likely to be necessary for sparse PCA with symmetric noise. In our proofs we use bounds on the covering numbers of sets of pseudo-expectations, which we obtain by certifying in sum-of-squares upper bounds on the Gaussian complexities of sets of solutions. This approach for bounding the covering numbers of sets of pseudo-expectations may be interesting in its own right and may find other application in future works.

==> content/ExpTime.tex <==
\section{Exponential-time algorithm}
\label{sec:expTime}
Before introducing our sum-of-squares algorithm, it will be conceptually helpful to describe an exponential-time algorithm containing several important ideas.
For every 3-tensor ${T}\in (\R^n)^{\otimes 3}$, define
\begin{align}\label{eq:tensorHuberLoss}
	F_h({T}):=\sum_{i,j,k\in [n]}f_h({T}_{ijk})\,,
\end{align}
where $f_h()$ is the Huber-penalty as defined in \cref{eq:huber-penalty}.
We prove that such estimator indeed recover the hidden vector $v\in \R^n$.
\begin{theorem}
	\label{thm:expTime}
	Let $0<\epsilon<1$, $\tau, \zeta>0$, $\displaystyle \alpha>\frac{4\sqrt{\ln(2)}}{\epsilon n}$ and $\displaystyle h=\frac{2\tau}{n^{3/2}}+\zeta$.  Then, given $\tau$ and  $\mathbf{T}=\tau\cdot v^{\otimes 3}+ \mathbf{N}$ where $v\in \Set{\tfrac{-1}{\sqrt{n}}\,,\tfrac{1}{\sqrt{n}}}^n$ and $\mathbf{N}$ is a 3-tensor with independent, symmetrically distributed entries such that $\bbP \Brac{\Abs{\mathbf{N}_{i,j,k}}\leq \zeta}\geq \alpha$, the estimator
	\begin{align}\label{eq:TEstimateExpTime}
		\hat{\mathbf{v}} = {\arg\min}_{x\in \Set{-\frac{1}{\sqrt{n}},+\frac{1}{\sqrt{n}}}}F_h\Paren{\mathbf{T}-\tau x^{\otimes 3}}
	\end{align}
	satisfies
	\begin{equation*}
		\norm{v-\hat{\mathbf{v}}}\leq \min\left\{\epsilon,\frac{8h\sqrt{2n\ln(2)}}{\alpha\tau}\right\}
	\end{equation*}
	with probability $1-o(1)$.
\end{theorem}

The proof of \cref{thm:expTime} relies on a bound on the gradient of $F_h(\mathbf{N})$ and on the local curvature of the function in a ring around the true solution.
Concretely, we will use the following two intermediate steps.

\begin{lemma}[Local strong convexity]
	\label[lemma]{lem:strongConvexity}
	Consider the settings of \cref{thm:expTime} 
	%$\Delta\in (\R^n)^{\otimes 3}$.
	Then, with probability $1-o(1)$, for any $v\in \R^d$ satisfying $\Norm{x-v}\geq \eps$,
	\begin{equation*}
		F_h(\mathbf{N}+\tau(\tensorpower{v}{3}-\tensorpower{x}{3}))\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\tensorpower{v}{3}-\tensorpower{x}{3}} + \frac{\tau^2\cdot \alpha}{4}\Normf{\tensorpower{v}{3}-\tensorpower{x}{3}}^2\,.
		%\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2 \,.
	\end{equation*}
\end{lemma}

\begin{lemma}[Gradient bound]
	\label[lemma]{lem:gradBound}
	Consider the settings of \cref{thm:expTime}. Then, probability $1-o(1)$,
	\begin{equation*}
		\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\leq 2h\Normf{\Delta}\sqrt{n\ln(2)}\,,
	\end{equation*}
	for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$, where $\Delta:=v^{\otimes 3} - x^{\otimes 3}$.
\end{lemma}

We prove these lemmata in the subsequent sections and  obtain here \cref{thm:expTime}.

\begin{proof}[Proof of \cref{thm:expTime}]
	Define $\mathbf{\Delta} = v^{\otimes 3}-\hat{\mathbf{v}}^{\otimes 3}\,.$
	We may assume $\Norm{v-\mathbf{v}}>\eps$ since otherwise the Theorem statement is trivially satisfied.
	From \Cref{lem:strongConvexity}, we have
	\begin{align*}
		F_h(\mathbf{N}+\tau\mathbf{\Delta})\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}} +\frac{\tau^2\cdot \alpha}{4}\Normf{\mathbf{\Delta}}^2\,.% \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\mathbf{\Delta}_{ijk}^2 \\\,.
	\end{align*}
	On the other hand, since $\hat{\mathbf{v}}^{\otimes 3}$ is the minimizer in \eqref{eq:TEstimateExpTime}, it follows that
	\begin{equation*}
		F_h(\mathbf{N}+\tau\mathbf{\Delta})\leq F_h(\mathbf{N})\,,
	\end{equation*}
	and hence
	\begin{align*}
		\frac{\tau^2\cdot \alpha}{4}\Normf{\mathbf{\Delta}}\leq-\tau\cdot\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}\leq \tau\cdot|\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}|\leq 2h\cdot \tau \cdot \Normf{\mathbf{\Delta}}\sqrt{n\ln(2)}\,,
	\end{align*}
	where in the last step we used the gradient bound in \cref{lem:gradBound}.
	Rearranging we get
	\begin{equation*}
		\Normf{\mathbf{\Delta}}\leq \frac{8h\sqrt{n\ln(2)}}{\alpha\tau}\,.
	\end{equation*}
	Finally, the result follows observing that by  \cref{lem:normFTensorDiff} $\norm{v-\hat{\mathbf{v}}}\leq \sqrt{2}\Normf{\mathbf{\Delta}}\,.$
\end{proof}

\subsection{Bound on the gradient}
The proof of \cref{lem:gradBound} is straightforward.

\begin{proof}[Proof of \cref{lem:gradBound}]
	Fix $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ and let $\Delta:=v^{\otimes 3} - x^{\otimes 3}$. We have
	\begin{align*}
		\iprod{\nabla F_h(\mathbf{N}),\Delta} &= \sum_{ijk}f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}= \sum_{ijk}\mathbf{y}_{ijk}\,,
	\end{align*}
	where $\mathbf{y}_{ijk}:=f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}\,.$
	From the definition of the Huber-loss function, it is easy to see that $|f_h'(\mathbf{N}_{ijk})|\leq h$. Hence,
	\begin{equation*}
		|\mathbf{y}_{ijk}|\leq h\cdot\Delta_{ijk}\,.
	\end{equation*}
	On the other hand, since $\mathbf{N}_{ijk}$ is symmetrically distributed around zero, we have
	\begin{equation*}
		\E[\mathbf{y}_{ijk}]=\E[f_h'(\mathbf{N}_{ijk})]\cdot\Delta_{ijk}=0\cdot\Delta_{ijk}=0\,.
	\end{equation*}
	It follows from Hoeffding's inequality that
	\begin{align*}
		\Pr[\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq t] &\leq 2\exp\left(-\frac{2 t^2}{\sum_{i,j,k}(2h\cdot\Delta_{ijk})^2}\right)\\
		&=2\exp\left(-\frac{t^2}{2h^2\Normf{\Delta}^2}\right)
	\end{align*}
	and by taking $t=2h\Normf{\Delta}\sqrt{n\ln(2)}$, we get
	\begin{align*}
		\Pr[\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq 2h\Normf{\Delta}\sqrt{n\ln(2)}] &\leq 2\exp(-2n\ln(2))=2\cdot 4^{-n}\,.
	\end{align*}
	Now by applying a union bound over $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$, we conclude that with probability at least
	\begin{equation*}
		1- 2^{n}\cdot 2\cdot 4^{-n}=1-2^{1-n}=1-o(1)\,,
	\end{equation*}
	we have
	\begin{equation*}
		\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\leq 2h\Normf{\Delta}\sqrt{n\ln(2)}\,,
	\end{equation*}
	for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$.
\end{proof}

\subsection{Local strong convexity}
We prove here \cref{lem:strongConvexity}. First notice that, due its quadratic part, the Huber loss function satisfies a strong convexity property.

\begin{lemma}\label{lem:strongConvexityPropertyHuberLoss}
	Consider the settings of \cref{thm:expTime}. Let $x\in \Set{\frac{-1}{\sqrt{n}}, \frac{+1}{\sqrt{n}}}^n$ and $\Delta:=\tensorpower{v}{3}-\tensorpower{x}{3}$. For $\displaystyle h=\frac{2\tau}{n^{3/2}}+\zeta$, we have
		\begin{equation*}
			F_h(\mathbf{N}+\tau\Delta)\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\Delta} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2 \,.
		\end{equation*}
	\begin{proof}
		Using \cref{lem:second-order-behavior-huber}, 
		\begin{align*}
			&F_h(\mathbf{N}+\tau\Delta)\\
			&=\sum_{i,j,k\in [n]}f_h(\mathbf{N}_{ijk}+\tau\Delta_{ijk})\\
			&\geq \sum_{i,j,k\in [n]}\left(f_h(\mathbf{N}_{ijk})+f_h'(\mathbf{N}_{ijk})\cdot\tau\cdot\Delta_{ijk} + \frac{(\tau\cdot\Delta_{ijk})^2}{2}\ind{\abs{\mathbf{N}_{ijk}}\leq \zeta}\cdot \ind{\Abs{\tau\Delta_{ijk}}\leq h-\zeta}\right)\\
			&= F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\Delta} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2\,,
		\end{align*}
		where the last equality follows from the fact that
		$\Delta_{ijk}=v_iv_jv_k-x_ix_jx_k\in\left\{\frac{-2}{n^{3/2}},0,\frac{2}{n^{3/2}}\right\}$, which implies that
		\begin{align*}
			|\tau\Delta_{ijk}|\leq \frac{2\tau}{n^{3/2}}=h-\zeta\,.
		\end{align*}
	\end{proof}
\end{lemma}

We can now obtain the Lemma.
\begin{proof}[Proof of \cref{lem:strongConvexity}]
	By \cref{lem:strongConvexityPropertyHuberLoss} it suffices to show that with probability $1-o(1)$, for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ satisfying $\norm{x-v}\geq \epsilon$ we have
	\begin{equation*}
		\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
	\end{equation*}
	where  $\Delta:=v^{\otimes 3} - x^{\otimes 3}$.
	To this end fix such an $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$.
	For every $i,j,k\in[n]$, define the random variable
	\begin{equation*}
		\mathbf{z}_{ijk} := \Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\,,
	\end{equation*}
	and let
	\begin{equation*}
		\mathbf{z} = \sum_{i,j,k\in [n]} \mathbf{z}_{ijk}\,.
	\end{equation*}
	We have
	\begin{align*}
		\E[\mathbf{z}] &= \sum_{i,j,k\in [n]} \E[\mathbf{z}_{ijk}] = \sum_{i,j,k\in [n]} \Pr[|\mathbf{N}_{ijk}|\leq \zeta]\cdot \Delta_{ijk}^2\geq \sum_{i,j,k\in [n]} \alpha\cdot \Delta_{ijk}^2=\alpha\cdot\normf{\Delta}^2\,.
	\end{align*}
	On the other hand, since $0\leq \mathbf{z}_{ijk}\leq \Delta_{ijk}^2$ for all $i,j,k\in[n]$, it follows from Hoeffding's inequality that for every $t>0$, we have
	\begin{align*}
		\Pr[\mathbf{z}-\E[\mathbf{z}]\leq -t] &\leq \exp\left(-\frac{2 t^2}{\sum_{i,j,k}\Delta_{ijk}^4}\right)\\
		&\stackrel{\text{(a)}}=\exp\left(-\frac{2 t^2}{\frac{4}{n^3}\sum_{i,j,k}\Delta_{ijk}^2}\right)=\exp\left(-\frac{n^3 t^2}{2\normf{\Delta}^2}\right)\,.
	\end{align*}
	where (a) follows from the fact that $\Delta_{ijk}=v_iv_jv_k-x_ix_jx_k\in\left\{\frac{-2}{n^{3/2}},0,\frac{2}{n^{3/2}}\right\}$, which means that $\Delta_{ijk}^4 = \frac{4}{n^3}\Delta_{ijk}^2$. By taking $t=\frac{\alpha}{2}\normf{\Delta}^2$, we get
	\begin{align*}
		\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] &= \Pr\left[\mathbf{z}-\E[\mathbf{z}]\leq -\frac{\alpha}{2}\normf{\Delta}^2\right]\leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8}\right)\,.
	\end{align*}
	Now since $\norm{x-v}\geq \epsilon$ and both vectors are flat, we know from \Cref{lem:normFTensorDiff} that $\normf{\Delta}\geq \frac{1}{\sqrt{2}}\norm{x-v}\geq \frac{\epsilon}{\sqrt{2}}$. Therefore,
	\begin{align*}
		\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] \leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8}\right)\leq \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16}\right)\,.
	\end{align*}
	Using the union bound, we conclude that with probability at least
	\begin{align*}
		1-2^n\cdot \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16}\right)=1- \exp\left(n\ln(2)-\frac{n^3 \alpha^2\epsilon^2}{16}\right)\,,
	\end{align*}
	we have
	\begin{equation*}
		\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
	\end{equation*}
	for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ satisfying $\norm{x-v}\geq \epsilon$. By setting $\alpha>\frac{4\sqrt{\ln(2)}}{\epsilon n}\,,$	we get the lemma.
\end{proof}




==> content/other-applications.tex <==
\subsection{Oblivious (sparse) linear regression}\label{section:obliviousRegression}
\todo

\Gnote{do we need it?}
\subsection{Oblivious principal component analysis}\label{section:ObliviousPCA}
\todo

\Gnote{do we need it?}

==> content/tensor-pca-without-meta.tex <==
\section{Tensor PCA (without meta-theorem)}


Let $t\in \N$ be such that $t\ge 6$ and let $b > 0$. Denote by $\cP_{b,t}$ the set of pseudo-distributions of degree $t$ over variables $x\in \R^n$ which satisfy the constraints 
\[
\mathcal{A}_b=\Set{x_i^2 \leq \frac{b^2}n:\forall i\in[n]}\cup\Set{\|x\|^2=1}\,.
\]

Denote

\[
\Omega_{b,t} = \Set{\pE x^{\otimes 3}  \suchthat \pE \in \cP_{b,t}(x)}\,.
\]

Note that this set is convex. Furthermore, for every \(X\in \Omega_{b,t}\), we have \(\Abs{X_{ijk}}\leq \frac{b^3}{n^{3/2}}\). Indeed, if \(\pE \in \cP_{b,t}(x)\) is such that \(X = \pE x^{\otimes 3}\), then
\[\Abs{X_{ijk}} = \Abs{\pE x_ix_jx_k} \stackrel{(\ast)}\leq \sqrt{\Paren{\pE x_i^2}\Paren{\pE x_j^2x_k^2}}\stackrel{(\dagger)}\leq \sqrt{\Paren{\frac{b^2}n}\Paren{\frac{b^4}{n^2}}}=\frac{b^3}{n^{3/2}}\,,\]
where \((\ast)\) follows from SOS Cauchy-Schwarz inequality and \((\dagger)\) follows from the fact that \(\mathcal{A}_b\) contains \(\Set{x_i^2 \leq \frac{b^2}n,~x_j^2 \leq \frac{b^2}n,~x_k^2 \leq \frac{b^2}n}\), which implies that \(\mathcal{A}_b\sststile{t}{} \Set{x_i^2\leq \frac{b^2}{n},~x_j^2\cdot x_k^2\leq \frac{b^2}{n}\cdot\frac{b^2}{n}}\).

Now let \(\tau,\zeta>0\) and \(0<\alpha<1\). Let \(v\in\R^n\) be an unknown unit vector satisfying \(v_i^2\leq\frac{b^2}{n}\) for all \(i\in[n]\), and let
\[\mathbf{T} = \tau v^{\otimes 3}+\mathbf{N}\,,\]
where the entries \(\Paren{\mathbf{N}_{ijk}}_{i,j,k\in[n]}\) of the tensor \(\mathbf{N}\) are independent, have symmetric distributions, and satisfy \(\Pr\Brac{\Abs{\mathbf{N}_{ijk}}\leq \zeta}\geq \alpha\) for all \(i,j,k\in[n]\). We observe \(\mathbf{T}\) and we would like to estimate \(v\). In order to do so, let \(h>0\) (to be determined later) and consider the following convex optimization problem:

\begin{equation}\label{eq:ConvexProblem_wmt}
\minimize_{X\in \Omega_{b,t}} F_h(\mathbf{T} - \tau X)\,.
\end{equation}

We claim that for an appropriate choice of \(h\), the above convex program yields a tensor \(\hat{\mathbf{X}}=\text{argmin}_{X\in \Omega_{b,t}}F_h(\mathbf{T} - \tau X)\) which is a good approximation of \(v^{\otimes 3}\). We will later show how we can extract from \(\hat{\mathbf{X}}\) a vector \(\hat{\mathbf{v}}\in\R^n\) that estimates \(v\).

%In order to study the convex program in \eqref{eq:ConvexProblem__wmt}, we need a few definitions and lemmas.
%
%Let us first introduce some useful notation. We define the two matrices \(I_{n^2},I_{n,n}\in (\R^n)^{\otimes 2}\times (\R^n)^{\otimes 2}\) as follows:
%\[\Paren{I_{n^2}}_{(i,j),(k,l)}=
%\begin{cases}
%1\quad&\text{if }i=k\text{ and }j=l\,,\\ 
%0\quad&\text{otherwise},
%\end{cases}
%\]
%and
%\[\Paren{I_{n,n}}_{(i,j),(k,l)}=
%\begin{cases}
%1\quad&\text{if }i=j\text{ and }k=l\,,\\ 
%0\quad&\text{otherwise}.
%\end{cases}
%\]
%
%Notice that \(I_{n^2}\) is just the identity matrix

\begin{definition}
Let \(A\in(\R^n)^{\otimes 3}\) be a 3-order tensor and let \(A_1,\ldots,A_n\in\R^{n\times n}\) be its slices in the first mode, i.e., for all \(u,v,w\in \R^n\), we have \[\Iprod{A,u\otimes v\otimes w}=\sum_{i=1}^n u_i \Iprod{v,A_i w}\,.\]

We say that the tensor \(A\) is \(\lambda\)-\emph{bounded} if
\[\sum_{i=1}^n A_i\otimes A_i \preceq \lambda^2\cdot M\,,\]
where \(M\in (\R^n)^{\otimes 2}\times (\R^n)^{\otimes 2}\) is any matrix that satisfies
\[\Iprod{u\otimes v,M\cdot(u\otimes v)}=\Iprod{u,v}^2,\quad\forall u,v\in\R^{n}\,.\]
\end{definition}

The following fact is an immediate corollary of the above definition:

\begin{lemma}
If \(A\in(\R^n)^{\otimes 3}\) is \(\lambda\)-bounded, then
\end{lemma}
\begin{proof}

\end{proof}

The following lemma is a generalization of \cite[Theorem 11]{DBLP:conf/colt/HopkinsSS15} to subgaussian entries:

\begin{lemma}
\label{lem:subGaussianTensor_wmt}
If \(\mathbf{A}\in (\R^n)^{\otimes 3}\) is a random 3-order tensor such that its entries \(\Paren{\mathbf{A}_{ijk}}_{i,j,k\in[n]}\) are independent and 1-subgaussian, then with probability \(1-o(1)\), the tensor \(\mathbf{A}\) is \(\lambda\)-bounded for \(\lambda = O(n^{3/4}(\log n)^{1/4})\).
\end{lemma}
\begin{proof}
The proof has a very similar structure to that of \cite[Theorem 11]{DBLP:conf/colt/HopkinsSS15}. We just need to use concentration bounds for matrices with independent subgaussian entries instead of those for matrices with i.i.d. Gaussian entries.
\end{proof}


Denote by $\Card{\cN_\eps(\Omega_{b,t})}$ the size of the minimal $\eps$-net in  $\Omega_{b,t}$.

\begin{lemma}[Gradient bound]
	\label[lemma]{lem:gradBoundSoS_wmt}
	With probability $1-o(1)$, for every $X\in \Omega_{b,t}$.
	\begin{equation*}
	\Abs{\iprod{\nabla F_h(\mathbf{N}), v^{\otimes 3} - X}}\leq 10h\Normf{v^{\otimes 3} - X}\sqrt{\ln\Card{\cN_\eps(\Omega_{b,t})}}\,.
	\end{equation*}
\end{lemma}
\begin{proof}
		Define \(\mathbf{A}:=\nabla F_h(\mathbf{N})\). For every \(i,j,k\in[n]\), we have
		\[\mathbf{A}_{i,j,k}=f_h'(\mathbf{N}_{ijk})\,,\]
hence, the entries of \(\mathbf{A}\) are independent. Furthermore, from the definition of the Huber-loss function, it is easy to see that $|f_h'(\mathbf{N}_{ijk})|\leq h$. We conclude that the entries of \(\mathbf{A}\) are \(h\)-subgaussian. It follows from \Cref{lem:subGaussianTensor_wmt} that with probability \(1-o(1)\), the tensor \(\mathbf{A}\) is \(\lambda\)-bounded, where
\[\lambda = O\Paren{h\cdot n^{3/4}(\log n)^{1/4}}\,.\]
		
		Now fix $X\in \Omega_{b,t}$ and let \(\pE\in\mathcal{P}_{b,t}\) be such that \(X=\pE x^{\otimes 3}\). Let \(\mathbf{A}_1,\ldots,\mathbf{A}_n\in\R^{n\times n}\) be the slices of \(\mathbf{A}\) in the first mode . We have
	\begin{align*}
	\Abs{\iprod{\nabla F_h(\mathbf{N}),v^{\otimes 3} - X}} &= \Abs{\pE\Iprod{\mathbf{A}, v^{\otimes 3} - x^{\otimes 3}}}\\
	&\leq \Abs{\pE\Iprod{\mathbf{A}, (v-x)\otimes v\otimes v}}+\Abs{\pE\Iprod{\mathbf{A}, x\otimes (v-x)\otimes v}}+\Abs{\pE\Iprod{\mathbf{A}, x\otimes x\otimes (v-x)}}\,.
	\end{align*}
	
	In the following, we analyze each of the above three terms:
	
\begin{align*}
\Abs{\pE\Iprod{\mathbf{A}, (v-x)\otimes v\otimes v}} &= \Abs{\sum_{i\in [n]}\pE(v-x)_i\Iprod{v, \mathbf{A}_i v}}\\
&\leq \Norm{v-\pE x} \cdot \sqrt{\sum_{i\in [n]}\Iprod{v, \mathbf{A}_i v}^2}
\end{align*}	
	
	
		
%		 We have
%	\begin{align*}
%	\iprod{\nabla F_h(\mathbf{N}),\Delta} &= \sum_{ijk}f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}= \sum_{ijk}\mathbf{y}_{ijk}\,,
%	\end{align*}
%	where $\mathbf{y}_{ijk}:=f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}\,.$
%	From the definition of the Huber-loss function, it is easy to see that $|f_h'(\mathbf{N}_{ijk})|\leq h$. Hence,
%	\begin{equation*}
%	|\mathbf{y}_{ijk}|\leq h\cdot\Delta_{ijk}\,.
%	\end{equation*}
%	On the other hand, since $\mathbf{N}_{ijk}$ is symmetrically distributed around zero, we have
%	\begin{equation*}
%	\E[\mathbf{y}_{ijk}]=\E[f_h'(\mathbf{N}_{ijk})]\cdot\Delta_{ijk}=0\cdot\Delta_{ijk}=0\,.
%	\end{equation*}
%	It follows from Hoeffding's inequality that
%	\begin{align*}
%	\Pr\Brac{\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq t} &\leq 2\exp\Paren{-\frac{2 t^2}{\sum_{i,j,k}(2h\cdot\Delta_{ijk})^2}}\\
%	&=2\exp\Paren{-\frac{t^2}{2h^2\Normf{\Delta}^2}}
%	\end{align*}
%	and by taking $t=10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega_{b,t})}}$, we get
%	\begin{align*}
%	\Pr\Brac{\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq 10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega_{b,t})}}} &\leq \Card{\cN_\eps(\Omega_{b,t})}^{-10}\,.
%	\end{align*}
%	The result follows using union bound over $X\in \Omega_{b,t}$.
\end{proof}

\begin{lemma}
\label{lem:normFTensorDiffSoS_wmt} Let \(v\in\R^n\) be a unit vector and let \(\pE\) be a pseudodistribution on the \(n\) formal variables \(x_1,\ldots,x_n\) satisfying \(\pE\Norm{x}^2 = \pE\Brac{x_1^2+\ldots+x_n^2}=1\). We have
\[\frac{1}{2}\pE\norm{v-x}^2\leq \pE\normf{\Delta}^2\]

 of \eqref{eq:polynomialConstraints}, there is a degree-6 sum-of-squares proof of the following inequalities
\begin{equation}
\mathcal{A}\vdash_6 \frac{1}{2}\norm{v-x}^2\leq \normf{\Delta}^2\leq 10\norm{v-x}^2\,.
\end{equation}
\end{lemma}
\begin{proof}
Using the triangular inequality, we have
\begin{align}
\mathcal{A}\vdash_6 \normf{\Delta}^2&=\Normf{v^{\otimes 3} - x^{\otimes 3}}^2\\
&\leq 2\Normf{v^{\otimes 3} - x\otimes v^{\otimes 2}}^2+2\Normf{x\otimes v^{\otimes 2} - x^{\otimes 3}}^2\\
&\leq 2\Normf{v^{\otimes 3} - x\otimes v^{\otimes 2}}^2+4\Normf{x\otimes v^{\otimes 2} - x^{\otimes 2}\otimes v }^2+4\Normf{x^{\otimes 2}\otimes v - x^{\otimes 3}}^2\\
&= 2\norm{v-x}^2\cdot\norm{v}^4+4\norm{x}^2\cdot\norm{v-x}^2\cdot\norm{v}^2+4\norm{x}^4\cdot\norm{v-x}^2\\
&= 10\norm{v-x}^2\,,
\end{align}
where in the last equality we used the fact that $v$ is a unit vector and that $\mathcal{A}\vdash_2 \norm{x}^2=1$. For the lower bound, we have
\begin{align}
\mathcal{A}\vdash_6 \normf{\Delta}^2&=\Normf{v^{\otimes 3}}^2 + \Normf{x^{\otimes 3}}^2 - 2\iprod{v^{\otimes 3},x^{\otimes 3}}=2 - 2\iprod{v,x}^3\\
&= (2-2\iprod{v,x})\cdot\left(1+\iprod{v,x}+\iprod{v,x}^2\right)\\
&\stackrel{\text{(a)}}= (\norm{v}^2 + \norm{x}^2-2\iprod{v,x})\cdot\left(1+\iprod{v,x}+\iprod{v,x}^2\right)\\
&\stackrel{\text{(b)}}\geq \norm{v-x}^2\cdot \frac{1}{2}\,,
\end{align}
where (a) follows from the fact that $v$ is a unit vector and $\mathcal{A}\vdash_2 \norm{x}^2=1$. (b) follows from the fact that
\begin{equation}
(1+t+t^2) - \frac{1}{2} = \Paren{t+\frac{1}{2}}^2+\left(\frac{1}{2}\right)^2\,.
\end{equation}
\end{proof}

\begin{lemma}[Local strong convexity]
	\label[lemma]{lem:strongConvexitySoS_wmt}
	%$\Delta\in (\R^n)^{\otimes 3}$.
	With probability $1-o(1)$, for every $X\in \Omega_{b,t}$ and for any $v\in \R^d$ satisfying $\Norm{X-v^{\otimes 3}}\geq \eps$,
	\begin{equation*}
	F_h(\mathbf{N}+\tau(\tensorpower{v}{3}-X))\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\tensorpower{v}{3}-X} + \frac{\tau^2\cdot \alpha}{4}\Normf{\tensorpower{v}{3}-X}^2\,.
	%\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2 \,.
	\end{equation*}
\end{lemma}

\begin{proof}
			Using \cref{lem:second-order-behavior-huber}, 
	\begin{align*}
	&F_h(\mathbf{N}+\tau\Delta)\\
	&=\sum_{i,j,k\in [n]}f_h(\mathbf{N}_{ijk}+\tau\Delta_{ijk})\\
	&\geq \sum_{i,j,k\in [n]}\left(f_h(\mathbf{N}_{ijk})+f_h'(\mathbf{N}_{ijk})\cdot\tau\cdot\Delta_{ijk} + \frac{(\tau\cdot\Delta_{ijk})^2}{2}\ind{\abs{\mathbf{N}_{ijk}}\leq \zeta}\cdot \ind{\Abs{\tau\Delta_{ijk}}\leq h-\zeta}\right)\\
	&= F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\Delta} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2\,,
	\end{align*}
	where the last equality follows from the fact that
	$\Abs{\Delta_{ijk}}\le \Abs{v_iv_jv_k} + \Abs{X_{ijk}}\le 2b^3/n^{3/2}$, which implies that
	\begin{align*}
	|\tau\Delta_{ijk}|\leq \frac{2b^3\tau}{n^{3/2}}=h-\zeta\,.
	\end{align*}
	So it suffices to show that with probability $1-o(1)$, for every $X\in \Omega_{b,t}$ satisfying $\norm{x-v}\geq \epsilon$ we have
	\begin{equation*}
	\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
	\end{equation*}
	where  $\Delta:=v^{\otimes 3} - X$.
	To this end fix such an $X\in \Omega_{b,t}$.
	For every $i,j,k\in[n]$, define the random variable
	\begin{equation*}
	\mathbf{z}_{ijk} := \Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\,,
	\end{equation*}
	and let
	\begin{equation*}
	\mathbf{z} = \sum_{i,j,k\in [n]} \mathbf{z}_{ijk}\,.
	\end{equation*}
	We have
	\begin{align*}
	\E[\mathbf{z}] &= \sum_{i,j,k\in [n]} \E[\mathbf{z}_{ijk}] = \sum_{i,j,k\in [n]} \Pr[|\mathbf{N}_{ijk}|\leq \zeta]\cdot \Delta_{ijk}^2\geq \sum_{i,j,k\in [n]} \alpha\cdot \Delta_{ijk}^2=\alpha\cdot\normf{\Delta}^2\,.
	\end{align*}
	On the other hand, since $0\leq \mathbf{z}_{ijk}\leq \Delta_{ijk}^2$ for all $i,j,k\in[n]$, it follows from Hoeffding's inequality that for every $t>0$, we have
	\begin{align*}
	\Pr[\mathbf{z}-\E[\mathbf{z}]\leq -t] &\leq \exp\left(-\frac{2 t^2}{\sum_{i,j,k}\Delta_{ijk}^4}\right)\\
	&\stackrel{\text{(a)}}\le\exp\left(-\frac{2 t^2}{\frac{4b^6}{n^3}\sum_{i,j,k}\Delta_{ijk}^2}\right)=\exp\left(-\frac{n^3 t^2}{2b^6\normf{\Delta}^2}\right)\,.
	\end{align*}
	where (a) follows from the fact that $\Abs{\Delta_{ijk}}\le 2b^3/n^{3/2}$, which means that $\Delta_{ijk}^4 \le \frac{4b^3}{n^3}\Delta_{ijk}^2$. By taking $t=\frac{\alpha}{2}\normf{\Delta}^2$, we get
	\begin{align*}
	\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] &\le \Pr\left[\mathbf{z}-\E[\mathbf{z}]\leq -\frac{\alpha}{2}\normf{\Delta}^2\right]\leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8b^3}\right)
	\leq \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16b^3}\right)\,.
	\end{align*}
	%Now since $\norm{x-v}\geq \epsilon$ and both vectors are flat, we know from \Cref{lem:normFTensorDiff} that $\normf{\Delta}\geq \frac{1}{\sqrt{2}}\norm{x-v}\geq \frac{\epsilon}{\sqrt{2}}$. 
%	Therefore,
%	\begin{align*}
%	\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] \leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8}\right)\leq \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16}\right)\,.
%	\end{align*}
	Using the union bound, we conclude that with probability at least
	\begin{align*}
	1-\Card{\cN_\eps(\Omega_{b,t})}\cdot \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16b^3}\right) \ge 1-o(1)
	\end{align*}
	we have
	\begin{equation*}
	\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
	\end{equation*}
	for every $X\in \Omega_{b,t}$ satisfying $\norm{X-v^{\otimes 3}}\geq \epsilon$. By setting $\alpha\gtrsim\frac{b^{3/2}}{\eps}\cdot\frac{\sqrt{\ln\Paren{\Card{\cN_\eps(\Omega_{b,t})}}}}{n^{3/2}} \,,$	we get the lemma.
\end{proof}

\begin{lemma}\label[lemma]{lem:epsNet_wmt}\
	For some absolute constant $C>0$,
	\[
	\Card{\cN_\eps(\Omega_{b,t})} \le \exp\Brac{\frac{C}{\eps^2}\cdot n^{3/2} \sqrt{\ln n}}\,.
	\]
\end{lemma}

\begin{proof}
	Let $\bm W \in \R^{n^3}$ be a tensor with \iid entries from $N(0,1)$. By \cref{fact:injectiveNormCertificate}, for all pseudo-distributions of degree $\ge 4$ such that $\pE_{\mu} \norm{x}^2 = 1$, 
	\[
	\pE\iprod{x^{\otimes 3}, \bm W} \le O\Paren{n^{3/4} \Paren{\ln n}^{1/4}}\,.
	\]
	
	Hence
	\[
	\sup_{X\in \Omega_{b,t}} \iprod{X,\bm W} \le O\Paren{n^{3/4} \Paren{\ln n}^{1/4}}\,.
	\]
	
	By \cref{fact:SudakovMinoration}, for all $\eps > 0$,
	\[
	\ln \Card{\cN_\eps(\Omega_{b,t})}  \le O\Paren{\frac{1}{\eps^2}\cdot n^{3/2} \sqrt{\ln n}}\,.
	\]
\end{proof}

\begin{theorem}[Main theorem]
	\label[lemma]{thm:MainTheorem_wmt}
    Let $0<\epsilon<1$, $\tau, \zeta, b>0$, $\displaystyle \alpha \gtrsim \frac{b^{3/2}}{\eps^2}\cdot \frac{\Paren{\ln n}^{1/4}}{ n^{3/4}}$ and $\displaystyle h=\frac{2b^3\tau}{n^{3/2}}+\zeta$.  Then, given $\tau$ and  $\mathbf{T}=\tau\cdot v^{\otimes 3}+ \mathbf{N}$ where $\abs{v_i}\le b/\sqrt{n}$ and $\mathbf{N}$ is a 3-tensor with independent, symmetrically distributed entries such that $\bbP \Brac{\Abs{\mathbf{N}_{i,j,k}}\leq \zeta}\geq \alpha$. 
    
    Then the estimator $\hat{\mathbf{v}} = \pE x$ satisfies
    \begin{equation*}
    \norm{v-\hat{\mathbf{v}}}\le O\Paren{\min\left\{\epsilon,\frac{h\cdot  n^{3/4}\Paren{\ln n}^{1/4}}{\eps\alpha \tau}\right\}}
    \end{equation*}
    with probability $1-o(1)$. 
\end{theorem}

\begin{proof}
	Define $\mathbf{\Delta} = v^{\otimes 3}-\hat{\mathbf{X}}\,.$
	We may assume $\Norm{v^{\otimes 3}-\hat{\mathbf{X}}}>\eps$ since otherwise the Theorem statement is satisfied by \cref{lem:normFTensorDiffSoS}.
	From \Cref{lem:strongConvexitySoS}, we have
	\begin{align*}
	F_h(\mathbf{N}+\tau\mathbf{\Delta})\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}} +\frac{\tau^2\cdot \alpha}{4}\Normf{\mathbf{\Delta}}^2\,.% \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\mathbf{\Delta}_{ijk}^2 \\\,.
	\end{align*}
	On the other hand, since $\hat{\mathbf{X}}$ is the minimizer in \eqref{eq:TEstimateExpTime}, it follows that
	\begin{equation*}
	F_h(\mathbf{N}+\tau\mathbf{\Delta})\leq F_h(\mathbf{N})\,,
	\end{equation*}
	and hence
	\begin{align*}
	\frac{\tau^2\cdot \alpha}{4}\Normf{\mathbf{\Delta}}^2\leq-\tau\cdot\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}\leq \tau\cdot|\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}|
	\leq \tau \cdot 10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega_{b,t})}}\,,
	\end{align*}
	where in the last step we used the gradient bound in \cref{lem:gradBoundSoS}.
	Rearranging we get
	\begin{equation*}
	\Normf{\mathbf{\Delta}}\leq \frac{40h\sqrt{\ln\Card{\cN_\eps(\Omega_{b,t})}}}{\alpha\tau} \le 
	O\Paren{\frac{h\cdot  n^{3/4}\Paren{\ln n}^{1/4}}{\eps\alpha \tau}}\,.
	\end{equation*}
	Finally, the result follows from \cref{lem:normFTensorDiffSoS}.
\end{proof}

==> content/tensor-pca.tex <==
\section{OLD proof}

\textbf{REMOVE EVERYTHING BELOW THIS POINT IN THE FILE}


\Tnote{To update from here}
Let $t\in \N$, $t\ge 6$ and $b > 0$. Denote by $\cP_t$ the set of pseudo-distributions of degree $t$ over variables $x\in \R^n$ which satisfy $\pE \norm{x}^2 = 1$. Denote by $\cC_b$ the set of tensors $X\in \R^{n^3}$ that satisfy  $\Abs{X_{ijk}}\le b^3/n^{3/2}$. Denote

\[
\Omega = \Set{X\in \cC_b \suchthat \exists \pE \in \cP_t(x), \pE x^{\otimes 3} = X }\,.
\]

Note that this set is convex.

Consider a convex optimization problem:

\begin{equation}\label{eq:ConvexProblem}
\minimize_{\substack{\pE\in\cP_t\\\pE x^{\otimes 3} \in \cC_b}} F_h(\bm T - \tau \pE x^{\otimes 3})\,.
\end{equation}

Denote by $\Card{\cN_\eps(\Omega)}$ the size of the minimal $\eps$-net in  $\Omega$.

\begin{lemma}[Gradient bound]
	\label[lemma]{lem:gradBoundSoS}
	With probability $1-o(1)$, for every $X\in \Omega$.
	\begin{equation*}
	\Abs{\iprod{\nabla F_h(\mathbf{N}), v^{\otimes 3} - X}}\leq 10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega)}}\,.
	\end{equation*}
\end{lemma}

\begin{proof}
		Fix $X\in \Omega$ and let $\Delta:=v^{\otimes 3} - X$. We have
	\begin{align*}
	\iprod{\nabla F_h(\mathbf{N}),\Delta} &= \sum_{ijk}f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}= \sum_{ijk}\mathbf{y}_{ijk}\,,
	\end{align*}
	where $\mathbf{y}_{ijk}:=f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}\,.$
	From the definition of the Huber-loss function, it is easy to see that $|f_h'(\mathbf{N}_{ijk})|\leq h$. Hence,
	\begin{equation*}
	|\mathbf{y}_{ijk}|\leq h\cdot\Delta_{ijk}\,.
	\end{equation*}
	On the other hand, since $\mathbf{N}_{ijk}$ is symmetrically distributed around zero, we have
	\begin{equation*}
	\E[\mathbf{y}_{ijk}]=\E[f_h'(\mathbf{N}_{ijk})]\cdot\Delta_{ijk}=0\cdot\Delta_{ijk}=0\,.
	\end{equation*}
	It follows from Hoeffding's inequality that
	\begin{align*}
	\Pr\Brac{\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq t} &\leq 2\exp\Paren{-\frac{2 t^2}{\sum_{i,j,k}(2h\cdot\Delta_{ijk})^2}}\\
	&=2\exp\Paren{-\frac{t^2}{2h^2\Normf{\Delta}^2}}
	\end{align*}
	and by taking $t=10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega)}}$, we get
	\begin{align*}
	\Pr\Brac{\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq 10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega)}}} &\leq \Card{\cN_\eps(\Omega)}^{-10}\,.
	\end{align*}
	The result follows using union bound over $X\in \Omega$.
\end{proof}

\begin{lemma}[Local strong convexity]
	\label[lemma]{lem:strongConvexitySoS}
	%$\Delta\in (\R^n)^{\otimes 3}$.
	With probability $1-o(1)$, for every $X\in \Omega$ and for any $v\in \R^d$ satisfying $\Norm{X-v^{\otimes 3}}\geq \eps$,
	\begin{equation*}
	F_h(\mathbf{N}+\tau(\tensorpower{v}{3}-X))\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\tensorpower{v}{3}-X} + \frac{\tau^2\cdot \alpha}{4}\Normf{\tensorpower{v}{3}-X}^2\,.
	%\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2 \,.
	\end{equation*}
\end{lemma}

\begin{proof}
			Using \cref{lem:second-order-behavior-huber}, 
	\begin{align*}
	&F_h(\mathbf{N}+\tau\Delta)\\
	&=\sum_{i,j,k\in [n]}f_h(\mathbf{N}_{ijk}+\tau\Delta_{ijk})\\
	&\geq \sum_{i,j,k\in [n]}\left(f_h(\mathbf{N}_{ijk})+f_h'(\mathbf{N}_{ijk})\cdot\tau\cdot\Delta_{ijk} + \frac{(\tau\cdot\Delta_{ijk})^2}{2}\ind{\abs{\mathbf{N}_{ijk}}\leq \zeta}\cdot \ind{\Abs{\tau\Delta_{ijk}}\leq h-\zeta}\right)\\
	&= F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\Delta} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2\,,
	\end{align*}
	where the last equality follows from the fact that
	$\Abs{\Delta_{ijk}}\le \Abs{v_iv_jv_k} + \Abs{X_{ijk}}\le 2b^3/n^{3/2}$, which implies that
	\begin{align*}
	|\tau\Delta_{ijk}|\leq \frac{2b^3\tau}{n^{3/2}}=h-\zeta\,.
	\end{align*}
	So it suffices to show that with probability $1-o(1)$, for every $X\in \Omega$ satisfying $\norm{x-v}\geq \epsilon$ we have
	\begin{equation*}
	\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
	\end{equation*}
	where  $\Delta:=v^{\otimes 3} - X$.
	To this end fix such an $X\in \Omega$.
	For every $i,j,k\in[n]$, define the random variable
	\begin{equation*}
	\mathbf{z}_{ijk} := \Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\,,
	\end{equation*}
	and let
	\begin{equation*}
	\mathbf{z} = \sum_{i,j,k\in [n]} \mathbf{z}_{ijk}\,.
	\end{equation*}
	We have
	\begin{align*}
	\E[\mathbf{z}] &= \sum_{i,j,k\in [n]} \E[\mathbf{z}_{ijk}] = \sum_{i,j,k\in [n]} \Pr[|\mathbf{N}_{ijk}|\leq \zeta]\cdot \Delta_{ijk}^2\geq \sum_{i,j,k\in [n]} \alpha\cdot \Delta_{ijk}^2=\alpha\cdot\normf{\Delta}^2\,.
	\end{align*}
	On the other hand, since $0\leq \mathbf{z}_{ijk}\leq \Delta_{ijk}^2$ for all $i,j,k\in[n]$, it follows from Hoeffding's inequality that for every $t>0$, we have
	\begin{align*}
	\Pr[\mathbf{z}-\E[\mathbf{z}]\leq -t] &\leq \exp\left(-\frac{2 t^2}{\sum_{i,j,k}\Delta_{ijk}^4}\right)\\
	&\stackrel{\text{(a)}}\le\exp\left(-\frac{2 t^2}{\frac{4b^6}{n^3}\sum_{i,j,k}\Delta_{ijk}^2}\right)=\exp\left(-\frac{n^3 t^2}{2b^6\normf{\Delta}^2}\right)\,.
	\end{align*}
	where (a) follows from the fact that $\Abs{\Delta_{ijk}}\le 2b^3/n^{3/2}$, which means that $\Delta_{ijk}^4 \le \frac{4b^3}{n^3}\Delta_{ijk}^2$. By taking $t=\frac{\alpha}{2}\normf{\Delta}^2$, we get
	\begin{align*}
	\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] &\le \Pr\left[\mathbf{z}-\E[\mathbf{z}]\leq -\frac{\alpha}{2}\normf{\Delta}^2\right]\leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8b^3}\right)
	\leq \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16b^3}\right)\,.
	\end{align*}
	%Now since $\norm{x-v}\geq \epsilon$ and both vectors are flat, we know from \Cref{lem:normFTensorDiff} that $\normf{\Delta}\geq \frac{1}{\sqrt{2}}\norm{x-v}\geq \frac{\epsilon}{\sqrt{2}}$. 
%	Therefore,
%	\begin{align*}
%	\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] \leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8}\right)\leq \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16}\right)\,.
%	\end{align*}
	Using the union bound, we conclude that with probability at least
	\begin{align*}
	1-\Card{\cN_\eps(\Omega)}\cdot \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16b^3}\right) \ge 1-o(1)
	\end{align*}
	we have
	\begin{equation*}
	\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
	\end{equation*}
	for every $X\in \Omega$ satisfying $\norm{X-v^{\otimes 3}}\geq \epsilon$. By setting $\alpha\gtrsim\frac{b^{3/2}}{\eps}\cdot\frac{\sqrt{\ln\Paren{\Card{\cN_\eps(\Omega)}}}}{n^{3/2}} \,,$	we get the lemma.
\end{proof}

\begin{lemma}\label[lemma]{lem:epsNet}\
	For some absolute constant $C>0$,
	\[
	\Card{\cN_\eps(\Omega)} \le \exp\Brac{\frac{C}{\eps^2}\cdot n^{3/2} \sqrt{\ln n}}\,.
	\]
\end{lemma}

\begin{proof}
	Let $\bm W \in \R^{n^3}$ be a tensor with \iid entries from $N(0,1)$. By \cref{fact:injectiveNormCertificate}, for all pseudo-distributions of degree $\ge 4$ such that $\pE_{\mu} \norm{x}^2 = 1$, 
	\[
	\pE\iprod{x^{\otimes 3}, \bm W} \le O\Paren{n^{3/4} \Paren{\ln n}^{1/4}}\,.
	\]
	
	Hence
	\[
	\sup_{X\in \Omega} \iprod{X,\bm W} \le O\Paren{n^{3/4} \Paren{\ln n}^{1/4}}\,.
	\]
	
	By \cref{fact:SudakovMinoration}, for all $\eps > 0$,
	\[
	\ln \Card{\cN_\eps(\Omega)}  \le O\Paren{\frac{1}{\eps^2}\cdot n^{3/2} \sqrt{\ln n}}\,.
	\]
\end{proof}

\begin{theorem}[Main theorem]
	\label[lemma]{thm:MainTheorem}
    Let $0<\epsilon<1$, $\tau, \zeta, b>0$, $\displaystyle \alpha \gtrsim \frac{b^{3/2}}{\eps^2}\cdot \frac{\Paren{\ln n}^{1/4}}{ n^{3/4}}$ and $\displaystyle h=\frac{2b^3\tau}{n^{3/2}}+\zeta$.  Then, given $\tau$ and  $\mathbf{T}=\tau\cdot v^{\otimes 3}+ \mathbf{N}$ where $\abs{v_i}\le b/\sqrt{n}$ and $\mathbf{N}$ is a 3-tensor with independent, symmetrically distributed entries such that $\bbP \Brac{\Abs{\mathbf{N}_{i,j,k}}\leq \zeta}\geq \alpha$. 
    
    Then the estimator $\hat{\mathbf{v}} = \pE x$ satisfies
    \begin{equation*}
    \norm{v-\hat{\mathbf{v}}}\le O\Paren{\min\left\{\epsilon,\frac{h\cdot  n^{3/4}\Paren{\ln n}^{1/4}}{\eps\alpha \tau}\right\}}
    \end{equation*}
    with probability $1-o(1)$. 
\end{theorem}

\begin{proof}
	Define $\mathbf{\Delta} = v^{\otimes 3}-\hat{\mathbf{X}}\,.$
	We may assume $\Norm{v^{\otimes 3}-\hat{\mathbf{X}}}>\eps$ since otherwise the Theorem statement is satisfied by \cref{lem:normFTensorDiffSoS}.
	From \Cref{lem:strongConvexitySoS}, we have
	\begin{align*}
	F_h(\mathbf{N}+\tau\mathbf{\Delta})\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}} +\frac{\tau^2\cdot \alpha}{4}\Normf{\mathbf{\Delta}}^2\,.% \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\mathbf{\Delta}_{ijk}^2 \\\,.
	\end{align*}
	On the other hand, since $\hat{\mathbf{X}}$ is the minimizer in \eqref{eq:TEstimateExpTime}, it follows that
	\begin{equation*}
	F_h(\mathbf{N}+\tau\mathbf{\Delta})\leq F_h(\mathbf{N})\,,
	\end{equation*}
	and hence
	\begin{align*}
	\frac{\tau^2\cdot \alpha}{4}\Normf{\mathbf{\Delta}}^2\leq-\tau\cdot\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}\leq \tau\cdot|\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}|
	\leq \tau \cdot 10h\Normf{\Delta}\sqrt{\ln\Card{\cN_\eps(\Omega)}}\,,
	\end{align*}
	where in the last step we used the gradient bound in \cref{lem:gradBoundSoS}.
	Rearranging we get
	\begin{equation*}
	\Normf{\mathbf{\Delta}}\leq \frac{40h\sqrt{\ln\Card{\cN_\eps(\Omega)}}}{\alpha\tau} \le 
	O\Paren{\frac{h\cdot  n^{3/4}\Paren{\ln n}^{1/4}}{\eps\alpha \tau}}\,.
	\end{equation*}
	Finally, the result follows from \cref{lem:normFTensorDiffSoS}.
\end{proof}
%
%\subsection{Decomposability of the sum-of-squares tensor nuclear norm}
%
%\begin{theorem}[Decomposatibilty of SoS tensor nuclear norm]\label{thm:decomposability-tensor-nuclear-norm}
%	Let $\Omega \subseteq \overline{\Omega}\subseteq \Paren{\R^{n}}^{\otimes 3}$. Then for any integer $t\geq 2$ and ${M}\in \Omega\,, {M'}\in \overline{\Omega}^{\bot}$
%	\begin{align*}
%		\Normns{{M}+{M'}}{t} = \Normns{{M}}{t}+ \Normns{{M'}}{t}\,.
%	\end{align*}
%\end{theorem}
%
%To prove \cref{thm:decomposability-tensor-nuclear-norm} we make use of the following intermediate step.
%
%\begin{lemma}\label{lem:support-pd-tensor-nuclear-norm}
%	Let $\Omega\subseteq \Paren{\R^n}^{\otimes 3}$ and let ${M}\in \Omega$. For any  $t\geq 2$, there exists ${A}\in \Omega$ such that $\Normins{{A}}{t}\leq 1$ and  
%	\begin{align*}
%		\Normns{{M}}{t}=\iprod{{M}, {A}}\,.
%	\end{align*}
%	\begin{proof}
%		The inner product is equivalent to $\iprod{{M}, {A}_{\Omega}}$, where ${A}_{\Omega}$ is the projection of ${A}$ onto $\Omega$.
%		\Tnote{To formally argue:} Since $\Normins{{A}_{\Omega}}{t}\leq \Normins{{A}}{t}$ the result follows.
%	\end{proof}
%\end{lemma}
%
%We can now prove decomposability.
%
%\begin{proof}[Proof of \cref{thm:decomposability-tensor-nuclear-norm}]
%	Since any norm satisfies  the triangle inequality, we only need to show 
%	\begin{align*}
%		\max_{\Normins{{A}}{t}\leq 1}\iprod{{M}+{M'}, {A}}\geq
%		\max_{\Normins{{B}}{t}\leq 1}\iprod{{M}, {B}} + \max_{\Normins{{C}}{t}\leq 1}\iprod{{M'}, {C}}\,.
%	\end{align*}
%	By \cref{lem:support-pd-tensor-nuclear-norm} we may assume
%	${B}\in \Omega$ and ${C}\in \overline{\Omega}^{\bot}$, thus we have 
%	\begin{align*}
%		\iprod{{M}+{M'}, {B} + {C}} = \Normns{{M}}{t} + \Normns{{M}'}{t}\,.
%	\end{align*}
%	It remains to argue that ${A}:={B}+{C}$ satisfies $\Normins{{A}}{t}\leq 1\,.$\Tnote{To check from here.}
%	
%	For a subspace $\Gamma\subseteq\Paren{\R^n}^{\otimes 3}$ We now introduce the notion of $\Gamma$-nice pseudo-distribution.
%	Consider a degree-$t$ pseudodistribution $\mu(x,y,z)$ satisfying $\pE\Norm{x}^2\,, \pE\Norm{y}^2\,, \pE\Norm{z}^2\leq 1$.	We may represent it as a block diagonal matrix $S^\mu$ with $\cS_{t/2, 3}$ \Tnote{Number of ways in which we can distribute $t/2$ balls in $3$ buckets} blocks each of size $n^{t/2}\times n^{t/2}$. \Rnote{Minor comment: We need to fix the notation so that we also consider monomial of degree $<t$.}
%	We can denote each block by $S^\mu_{t_x, t_y, t_z}$ where where $t_x+t_y+t_z=t/2$ and write any squared polynomial in indeterminates $x,y,z$ as 
%	$\iprod{x^{\otimes t_x}\otimes y ^{\otimes t_y}\otimes z^{\otimes t_z}, S^\mu_{t_x, t_y, t_z} x^{\otimes t_x}\otimes y^{\otimes{t_y}}\otimes z^{\otimes t_z}}$.
%	We construct now a new degree-$t$ pseudodistribution $\nu(x,y,z)$ as follows.
%	We construct a new block diagonal matrix $S^\nu$ with $\cS_{t/2, 3}$ blocks each of size $n^{t/2}\times n^{t/2}$. 
%	To show that $\nu$ is indeed a pseudo-distribution, it suffices to show that each such block $S^\nu_{t_x,t_y, t_z}$ is positive semidefinite.
%	We define each block as
%	\begin{align*}
%		S^\nu_{t_x,t_y, t_z} := \Pi_{\Gamma^{\otimes t/2}}S^\mu_{t_x, t_y, t_z}\Pi_{\Gamma^{\otimes t/2}}\,,
%	\end{align*}
%	where $\Pi_{\Gamma^{\otimes t/2}}$ is the orthogonal projector onto $\Gamma^{\otimes t/2}$. By definition $S^\nu_{t_x,t_y, t_z}\sge 0$ and for any ${Z}\in \Gamma$ we have 
%	\begin{align*}
%		\pE_\mu \iprod{{Z}, x\otimes y \otimes z} = \pE_\nu \iprod{{Z}, x\otimes y \otimes z}\,.
%	\end{align*}
%	Notice also that $\nu$ satisfies $\pE_\nu\Norm{x}^2\,, \pE_\nu\Norm{y}^2\,, \pE_\nu\Norm{z}^2\leq1$
%	We call pseudo-distributions constructed as $\nu$ $\Gamma$-\textit{nice} pseudo-distribution.
%	
%	%We can make a similar argument for $\mathbf{C}$ by changing the projector to $\Pi_{\Paren{\overline{\Omega}^{\bot}}^{\otimes t/2}}$.
%	Consider now  a new pseudo-distribution $\zeta$ satisfying $\pE\Norm{x}^2\,, \pE\Norm{y}^2\,,  \pE\Norm{z}^2\leq 1$.
%	We will construct a pseudo-distribution $\zeta'$ (still satisfying our constraints) such that
%	\begin{align*}
%		\pE_\zeta \iprod{{A}, x\otimes y\otimes z} = 	\pE_{\zeta'} \iprod{{A}, x\otimes y\otimes z}
%	\end{align*}
%	then we will show 
%	\begin{align*}
%		\pE_{\zeta'} \iprod{{A}, x\otimes y\otimes z}\leq 1\,.
%	\end{align*}
%	
%	We can encode $\zeta$ by a set of $\cS_{t/2,3}$ matrices $S^\zeta_{t_x,t_y, t_z}$ of size $n^{t/2}\times n^{t/2}$, where $t_x+t_y+t_z=t/2$.
%	Indeed we may write any squared polynomial of degree $t$ 
%	in indeterminates $x,y,z$ as 
%	$\iprod{x^{\otimes t_x}\otimes y ^{\otimes t_y}\otimes z^{\otimes t_z}, S^\zeta_{t_x, t_y, t_z} x^{\otimes t_x}\otimes y^{\otimes{t_y}}\otimes z^{\otimes t_z}}$.
%	We now define
%	\begin{align*}
%		S^{\zeta'}_{t_x,t_y, t_z} = \Pi_{\Paren{\overline{\Omega}^{\bot}}^{\otimes t/2}}S^{\zeta}_{t_x,t_y, t_z}\Pi_{\Paren{\overline{\Omega}^{\bot}}^{\otimes t/2}} + \Pi_{\Omega^{\otimes t/2}}S^{\zeta}_{t_x,t_y, t_z}\Pi_{\Omega^{\otimes t/2}}\,.
%	\end{align*}
%	By definition $S^{\zeta'}_{t_x,t_y, t_z} \sge 0$ moreover we have 
%	\begin{align*}
%		\pE_{\zeta'}\Snorm{x}\,,\pE_{\zeta'}\Snorm{y}\,, \pE_{\zeta'}\Snorm{z}\leq 1\,.
%	\end{align*}
%	
%	By construction $\zeta'$ can be written as a convex combination of a $\Omega$-nice  pseudo-distribution $\nu$ and a $\overline{\Omega}^\bot$-nice pseudo-distribution $\nu'$ \Rnote{We need to be careful here because we have three constraints on $\|x\|^2,\|y\|^2,\|z\|^2$ rather than one: How can we ensure that both $\nu$ and $\nu'$ satisfy all three constraints simultaneously? If I understand correctly, the argument here is that we first define $\overline{\nu}$ to be the one induced by $\Pi_{\Omega^{\otimes t/2}}S^{\zeta}_{t_x,t_y, t_z}\Pi_{\Omega^{\otimes t/2}}$ and $\overline{\nu}'$ to be the one induced by $\Pi_{\Paren{\overline{\Omega}^{\bot}}^{\otimes t/2}}S^{\zeta}_{t_x,t_y, t_z}\Pi_{\Paren{\overline{\Omega}^{\bot}}^{\otimes t/2}}$ so that $\zeta'=\overline{\nu}+\overline{\nu}'$ and then define $\nu$ and $\nu'$ to be scaled versions of $\overline{\nu}$ and $\overline{\nu}'$ so that $\zeta'$ becomes a convex combination of the scaled versions. However, we might not be able to find the scaling coefficients so that all the constraints are satisfied simultaneously: One can imagine a situation where $\pE_{\zeta'}\Snorm{x}=\pE_{\overline{\nu}}\Snorm{x}=1$ and $\pE_{\zeta'}\Snorm{y}=\pE_{\overline{\nu}'}\Snorm{y}=1$}.
%	Thus there is some $\gamma \in [0,1]$ such that
%	\begin{align*}
%		\pE_{\zeta'} \iprod{{A}, x\otimes y\otimes z} &\leq \gamma	\pE_{\nu} \iprod{{A}, x\otimes y\otimes z}  +(1-\gamma)\pE_{\nu'} \iprod{{A}, x\otimes y\otimes z} \\
%		&=  \gamma	\pE_{\nu} \iprod{{B}+{C}, x\otimes y\otimes z}  +(1-\gamma)\pE_{\nu'} \iprod{{B}+{C}, x\otimes y\otimes z} \\
%		&=  \gamma	\pE_{\nu} \iprod{{B}, x\otimes y\otimes z}  +(1-\gamma)\pE_{\nu'} \iprod{{C}, x\otimes y\otimes z} \leq 1\,.
%	\end{align*}
%	The result follows.
%\end{proof}

\section*{OLD FORMULATION}
In this section, we provide a polynomial-time algorithm that is based on sum-of-squares (SoS). We will essentially modify the estimator of \eqref{eq:TEstimateExpTime} in order to get a tractable algorithm.

First we introduce $n$ formal variables $x_1,\ldots,x_n$ satisfying the constraints
\begin{equation}
x_i^2 = \frac{1}{n}\,,\quad\text{for all }i\in[n]\,.
\end{equation}

Second, in order to use the sum-of-squares formalism, we need rewrite the estimator of \eqref{eq:TEstimateExpTime} using the language of polynomials. Even though the Huber-loss function itself is not a polynomial function, we can encode it using polynomial inequalities by introducing auxiliary variables: 
\begin{lemma}
\label[lemma]{lem:HuberLossRewritten}
For every $t,z\in\R$, we have $z=f_h(t)$ if and only if there exists $y\in \R$ such that:
\begin{itemize}
\item $y\geq 0$,
\item $y^2=t^2$,
\item $h\cdot y-\frac{h^2}{2}\leq z\leq \frac{y^2}{2}$,
\item $(h^2-y^2)\cdot\Paren{z-\frac{y^2}{2}}\geq 0$, and
\item $(y^2-h^2)\cdot\Paren{h\cdot y-\frac{h^2}{2}-z}\geq 0$.
\end{itemize}
\end{lemma}
\begin{proof}
It is easy to see that $z=f_h(t)$ and $y=|t|$ satisfy the five conditions of the lemma.

Conversely, if $t,z$ and $y$ satisfy the five conditions, then $y\geq 0$ and $y^2=t^2$ imply that $y=|t|$. Now we have three possibilities:
\begin{itemize}
\item If $|t|=y=h$, then $h\cdot y-\frac{h^2}{2}=\frac{h^2}{2}$ and $\frac{y^2}{2}=\frac{h^2}{2}$. The third condition then implies that $z=\frac{h^2}{2}=\frac{t^2}{2}=f_h(t)$.
\item If $|t|=y<h$, then $h^2-y^2>0$, and the fourth condition implies that $z\geq \frac{y^2}{2}$. By combining this with the third condition, we get $z=\frac{y^2}{2}=\frac{t^2}{2}=f_h(t)$.
\item If $|t|=y>h$, then $y^2-h^2>0$, and the fifth condition implies that $z\leq h\cdot y-\frac{h^2}{2}$. By combining this with the third condition, we get $z=h\cdot y-\frac{h^2}{2}=h\cdot |t|-\frac{h^2}{2}=f_h(t)$.
\end{itemize}
\end{proof}

Using \Cref{lem:HuberLossRewritten}, we can rewrite the estimator of \eqref{eq:TEstimateExpTime} in the language of polynomials as follows: For every $i,j,k\in[n]$, we introduce two formal variables $z_{ijk}$ and $y_{ijk}$, and the estimator becomes:

\begin{align}
\label{eq:TEstimateRewritten}\text{minimize} \quad& \sum_{i,j,k\in[n]} z_{ijk}\,,\quad \text{subject to } \mathcal{A}\,,
\end{align}
where $\mathcal{A}$ is a collection of polynomial equalities and inequalities defined as:
\begin{equation}
\label{eq:polynomialConstraints}
\mathcal{A}=\begin{Bmatrix*}[l]
x_i^2=\frac{1}{n}\,,\quad&\text{for all }i\in [n]\,,\\
y_{ijk}\geq 0~~\text{and}~~y_{ijk}^2=\left(\mathbf{T}_{ijk}-\tau x_ix_jx_k\right)^2\,,\quad&\text{for all }i,j,k\in [n]\,,\\
h\cdot y_{ijk}-\frac{h^2}{2}\leq z_{ijk}\leq \frac{y_{ijk}^2}{2} \,,\quad&\text{for all }i,j,k\in [n]\,,\\
\Paren{h^2-y_{ijk}^2}\cdot\Paren{z_{ijk}-\frac{y_{ijk}^2}{2}}\geq 0\,,\quad&\text{for all }i,j,k\in [n]\,,\\
\Paren{y_{ijk}^2-h^2}\cdot\Paren{h\cdot y_{ijk}-\frac{h^2}{2}-z_{ijk}}\geq0\,,\quad&\text{for all }i,j,k\in [n]
\end{Bmatrix*}
\end{equation}

The estimator in \eqref{eq:TEstimateRewritten} is still intractable. In order to make it tractable, we use the sum-of-squares formalism. We will search for a degree-4 pseudoexpectation 
\begin{equation}
\pE:\R\left[(x_i)_{i\in[n]},(y_{ijk})_{i,j,k\in[n]},(z_{ijk})_{i,j,k\in[n]}\right]_{\leq 4}\to\R\,,
\end{equation}
such that we minimize
\begin{align}
\sum_{i,j,k\in[n]} \pE[z_{ijk}]\,,\quad \text{subject to } \mathcal{A}\,,
\end{align}
After finding this pseudoexpectation, we output the unit vector $\mathbf{v}\in \R^n$ defined as
\begin{equation}
\mathbf{v}_i = \pE[x_i]\,,\quad\text{for all }i\in[n]\,.
\end{equation}

In the following, we will show that if $\tau$ and $\alpha$ are not too small, the above estimator is a good one. We will need to prove SoS versions of \cref{lem:normFTensorDiff,lem:strongConvexity,lem:strongConvexityPropertyHuberLoss,lem:gradBound}. We define the formal 3-tensor $\Delta$ as
\begin{align}
\Delta = v^{\otimes 3} - x^{\otimes 3}\,.
\end{align}

In the following, $\Delta_{ijk}$ is just an alias for the degree-3 polynomial $v_iv_jv_k - x_ix_jx_k$.


We first prove an SoS version of \cref{lem:normFTensorDiff}.

\begin{lemma}
\label[lemma]{lem:normFTensorDiffSoS} Given the constraints $\mathcal{A}$ of \eqref{eq:polynomialConstraints}, there is a degree-6 sum-of-squares proof of the following inequalities
\begin{equation}
\mathcal{A}\vdash_6 \frac{1}{2}\norm{v-x}^2\leq \normf{\Delta}^2\leq 10\norm{v-x}^2\,.
\end{equation}
\end{lemma}
\begin{proof}
Using the triangular inequality, we have
\begin{align}
\mathcal{A}\vdash_6 \normf{\Delta}^2&=\Normf{v^{\otimes 3} - x^{\otimes 3}}^2\\
&\leq 2\Normf{v^{\otimes 3} - x\otimes v^{\otimes 2}}^2+2\Normf{x\otimes v^{\otimes 2} - x^{\otimes 3}}^2\\
&\leq 2\Normf{v^{\otimes 3} - x\otimes v^{\otimes 2}}^2+4\Normf{x\otimes v^{\otimes 2} - x^{\otimes 2}\otimes v }^2+4\Normf{x^{\otimes 2}\otimes v - x^{\otimes 3}}^2\\
&= 2\norm{v-x}^2\cdot\norm{v}^4+4\norm{x}^2\cdot\norm{v-x}^2\cdot\norm{v}^2+4\norm{x}^4\cdot\norm{v-x}^2\\
&= 10\norm{v-x}^2\,,
\end{align}
where in the last equality we used the fact that $v$ is a unit vector and that $\mathcal{A}\vdash_2 \norm{x}^2=1$. For the lower bound, we have
\begin{align}
\mathcal{A}\vdash_6 \normf{\Delta}^2&=\Normf{v^{\otimes 3}}^2 + \Normf{x^{\otimes 3}}^2 - 2\iprod{v^{\otimes 3},x^{\otimes 3}}=2 - 2\iprod{v,x}^3\\
&= (2-2\iprod{v,x})\cdot\left(1+\iprod{v,x}+\iprod{v,x}^2\right)\\
&\stackrel{\text{(a)}}= (\norm{v}^2 + \norm{x}^2-2\iprod{v,x})\cdot\left(1+\iprod{v,x}+\iprod{v,x}^2\right)\\
&\stackrel{\text{(b)}}\geq \norm{v-x}^2\cdot \frac{1}{2}\,,
\end{align}
where (a) follows from the fact that $v$ is a unit vector and $\mathcal{A}\vdash_2 \norm{x}^2=1$. (b) follows from the fact that
\begin{equation}
(1+t+t^2) - \frac{1}{2} = \Paren{t+\frac{1}{2}}^2+\left(\frac{1}{2}\right)^2\,.
\end{equation}
\end{proof}

Next, we show an SoS proof of a strong convexity property that is satisfied by the Huber-loss function:

\begin{lemma}
\label[lemma]{lem:strongConvexitySoS-2}
For $\displaystyle h=\frac{2\tau}{n^{3/2}}+\zeta$, we have
\begin{equation}
\mathcal{A}\vdash_6 \sum_{i,j,k\in [n]} z_{ijk}\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\Delta} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2 \,.
\end{equation}
\end{lemma}
\begin{proof}
Using \cref{lem:second-order-behavior-huber}, we get

\begin{align}
&F_h(\mathbf{N}+\tau\Delta)\\
&=\sum_{i,j,k\in [n]}f_h(\mathbf{N}_{ijk}+\tau\Delta_{ijk})\\
&\geq \sum_{i,j,k\in [n]}\left(f_h(\mathbf{N}_{ijk})+f_h'(\mathbf{N}_{ijk})\cdot\tau\cdot\Delta_{ijk} + \frac{(\tau\cdot\Delta_{ijk})^2}{2}\ind{\abs{\mathbf{N}_{ijk}}\leq \zeta}\cdot \ind{\Abs{\tau\Delta_{ijk}}\leq h-\zeta}\right)\\
&= F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\Delta} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\Delta_{ijk}^2\,,
\end{align}
where the last equality follows from the fact that
$\Delta_{ijk}=v_iv_jv_k-x_ix_jx_k\in\left\{\frac{-2}{n^{3/2}},0,\frac{2}{n^{3/2}}\right\}$, which implies that
\begin{align}
|\tau\Delta_{ijk}|\leq \frac{2\tau}{n^{3/2}}=h-\zeta\,.
\end{align}
\end{proof}

%\begin{lemma}
%\label[lemma]{lem:frobNormBound}
%For every $0<\epsilon<1$, if $\displaystyle \alpha>\frac{4\sqrt{\ln(2)}}{\epsilon n}$, then with probability $1-o(1)$ we have
%\begin{equation}
%\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
%\end{equation}
%for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ satisfying $\norm{x-v}\geq \epsilon$, where $\Delta:=v^{\otimes 3} - x^{\otimes 3}$.
%\end{lemma}
%\begin{proof}
%Fix $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ satisfying $\norm{x-v}\geq \epsilon$, and let $\Delta:=v^{\otimes 3} - x^{\otimes 3}$. For every $i,j,k\in[n]$, define the random variable
%\begin{equation}
%\mathbf{z}_{ijk} := \Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\,,
%\end{equation}
%and let
%\begin{equation}
%\mathbf{z} = \sum_{i,j,k\in [n]} \mathbf{z}_{ijk}\,.
%\end{equation}
%
%We have
%\begin{align}
%\E[\mathbf{z}] &= \sum_{i,j,k\in [n]} \E[\mathbf{z}_{ijk}] = \sum_{i,j,k\in [n]} \Pr[|\mathbf{N}_{ijk}|\leq \zeta]\cdot \Delta_{ijk}^2\geq \sum_{i,j,k\in [n]} \alpha\cdot \Delta_{ijk}^2=\alpha\cdot\normf{\Delta}^2\,.
%\end{align}
%
%
%On the other hand, since $0\leq \mathbf{z}_{ijk}\leq \Delta_{ijk}^2$ for all $i,j,k\in[n]$, it follows from Hoeffding's inequality that for every $t>0$, we have
%\begin{align}
%\Pr[\mathbf{z}-\E[\mathbf{z}]\leq -t] &\leq \exp\left(-\frac{2 t^2}{\sum_{i,j,k}\Delta_{ijk}^4}\right)\\
%&\stackrel{\text{(a)}}=\exp\left(-\frac{2 t^2}{\frac{4}{n^3}\sum_{i,j,k}\Delta_{ijk}^2}\right)=\exp\left(-\frac{n^3 t^2}{2\normf{\Delta}^2}\right)\,.
%\end{align}
%where (a) follows from the fact that $\Delta_{ijk}=v_iv_jv_k-x_ix_jx_k\in\left\{\frac{-2}{n^{3/2}},0,\frac{2}{n^{3/2}}\right\}$, which means that $\Delta_{ijk}^4 = \frac{4}{n^3}\Delta_{ijk}^2$. By taking $t=\frac{\alpha}{2}\normf{\Delta}^2$, we get
%\begin{align}
%\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] &= \Pr\left[\mathbf{z}-\E[\mathbf{z}]\leq -\frac{\alpha}{2}\normf{\Delta}^2\right]\leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8}\right)\,.
%\end{align}
%
%Now since $\norm{x-v}\geq \epsilon$, we know from \Cref{lem:normFTensorDiff} that $\normf{\Delta}\geq \frac{1}{\sqrt{2}}\norm{x-v}\geq \frac{\epsilon}{\sqrt{2}}$. Therefore,
%\begin{align}
%\Pr\left[\mathbf{z}\leq \frac{\alpha}{2}\normf{\Delta}^2\right] \leq \exp\left(-\frac{n^3 \alpha^2\normf{\Delta}^2}{8}\right)\leq \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16}\right)\,.
%\end{align}
%
%Using the union bound, we conclude that with probability at least
%\begin{align}
%1-2^n\cdot \exp\left(-\frac{n^3 \alpha^2\epsilon^2}{16}\right)=1- \exp\left(n\ln(2)-\frac{n^3 \alpha^2\epsilon^2}{16}\right)\,,
%\end{align}
%we have
%\begin{equation}
%\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\cdot\Delta_{ijk}^2\geq \frac{\alpha}{2} \Normf{\Delta}^2\,,
%\end{equation}
%for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ satisfying $\norm{x-v}\geq \epsilon$. By setting
%\begin{align}
%\alpha>\frac{4\sqrt{\ln(2)}}{\epsilon n}\,,
%\end{align}
%we get the lemma.
%\end{proof}
%
%\begin{lemma}
%\label[lemma]{lem:gradBound}
%With probability $1-o(1)$ we have
%\begin{equation}
%\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\leq 2h\Normf{\Delta}\sqrt{n\ln(2)}\,,
%\end{equation}
%for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$, where $\Delta:=v^{\otimes 3} - x^{\otimes 3}$.
%\end{lemma}
%\begin{proof}
%Fix $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$ and let $\Delta:=v^{\otimes 3} - x^{\otimes 3}$. We have
%\begin{align*}
%\iprod{\nabla F_h(\mathbf{N}),\Delta} &= \sum_{ijk}f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}= \sum_{ijk}\mathbf{y}_{ijk}\,,
%\end{align*}
%where
%\begin{equation}
%\mathbf{y}_{ijk}:=f_h'(\mathbf{N}_{ijk})\cdot\Delta_{ijk}\,.
%\end{equation}
%From the definition of the Huber-loss function, it is easy to see that $|f_h'(\mathbf{N}_{ijk})|\leq h$. Hence,
%\begin{equation}
%|\mathbf{y}_{ijk}|\leq h\cdot\Delta_{ijk}\,.
%\end{equation}
%On the other hand, since $\mathbf{N}_{ijk}$ is symmetrically distributed around zero, we have
%\begin{equation}
%\E[\mathbf{y}_{ijk}]=\E[f_h'(\mathbf{N}_{ijk})]\cdot\Delta_{ijk}=0\cdot\Delta_{ijk}=0\,.
%\end{equation}
%It follows from Hoeffding's inequality that
%
%\begin{align}
%\Pr[\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq t] &\leq 2\exp\left(-\frac{2 t^2}{\sum_{i,j,k}(2h\cdot\Delta_{ijk})^2}\right)\\
%&=2\exp\left(-\frac{t^2}{2h^2\Normf{\Delta}^2}\right)\,.
%\end{align}
%
%By taking $t=2h\Normf{\Delta}\sqrt{n\ln(2)}$, we get
%\begin{align}
%\Pr[\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\geq 2h\Normf{\Delta}\sqrt{n\ln(2)}] &\leq 2\exp(-2n\ln(2))=2\cdot 4^{-n}\,.
%\end{align}
%Now by applying a union bound over $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$, we conclude that with probability at least
%\begin{equation}
%1- 2^{n}\cdot 2\cdot 4^{-n}=1-2^{1-n}=1-o(1)\,,
%\end{equation}
%we have
%\begin{equation}
%\Abs{\iprod{\nabla F_h(\mathbf{N}),\Delta}}\leq 2h\Normf{\Delta}\sqrt{n\ln(2)}\,,
%\end{equation}
%for every $x\in \left\{\frac{-1}{\sqrt{n}},\frac{+1}{\sqrt{n}}\right\}^n$.
%\end{proof}
%
%Now we are ready to prove that the estimator of \eqref{eq:TEstimateExpTime} is good
%
%\begin{theorem}
%\label{thm:expTime}
%Let $0<\epsilon<1$. If $\displaystyle \alpha>\frac{4\sqrt{\ln(2)}}{\epsilon n}$ and $\displaystyle h=\frac{2\tau}{n^{3/2}}+\zeta$, then with probability $1-o(1)$, the output $\hat{\mathbf{v}}$ of the estimator in \eqref{eq:TEstimateExpTime} satisfies
%\begin{equation}
%\norm{v-\hat{\mathbf{v}}}\leq \min\left\{\epsilon,\frac{8h\sqrt{n\ln(2)}}{\alpha\tau}\right\}\,.
%\end{equation}
%\end{theorem}
%\begin{proof}
%Define
%\begin{equation}
%\mathbf{\Delta} = v^{\otimes 3}-\hat{\mathbf{v}}^{\otimes 3}\,.
%\end{equation}
%
%From \Cref{lem:strongConvexity}, we have
%\begin{equation}
%F_h(\mathbf{N}+\tau\mathbf{\Delta})\geq F_h(\mathbf{N}) + \tau\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}} + \frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\mathbf{\Delta}_{ijk}^2 \,.
%\end{equation}
%
%On the other hand, since $\hat{\mathbf{v}}^{\otimes 3}$ is the minimizer in \eqref{eq:TEstimateExpTime}, it follows that
%\begin{equation}
%F_h(\mathbf{N}+\tau\mathbf{\Delta})\leq F_h(\mathbf{N})\,,
%\end{equation}
%and hence
%\begin{equation}
%\frac{1}{2}\sum_{i,j,k\in [n]}\Ind_{\{|\mathbf{N}_{ijk}|\leq \zeta\}}\tau^2\mathbf{\Delta}_{ijk}^2\leq -\tau\cdot\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}\leq \tau\cdot|\iprod{\nabla F_h(\mathbf{N}),\mathbf{\Delta}}|\,.
%\end{equation}
%
%Now since $\displaystyle \alpha>\frac{4\sqrt{\ln(2)}}{\epsilon n}$, it follows from \Cref{lem:frobNormBound} and \Cref{lem:gradBound} that with probability $1-o(1)$, we either have $\norm{v-\hat{\mathbf{v}}}< \epsilon$ or
%\begin{equation}
%\frac{1}{4}\alpha\tau\Normf{\mathbf{\Delta}}^2\leq 2h\Normf{\mathbf{\Delta}}\sqrt{n\ln(2)}\,.
%\end{equation}
%
%Note that if $\norm{v-\hat{\mathbf{v}}}\geq \epsilon$, the above implies that
%\begin{equation}
%\Normf{\mathbf{\Delta}}\leq \frac{8h\sqrt{n\ln(2)}}{\alpha\tau}\,.
%\end{equation}
%
%Now since \Cref{lem:normFTensorDiff} implies that $\norm{v-\hat{\mathbf{v}}}\leq \sqrt{2}\Normf{\mathbf{\Delta}}$, we conclude that
%\begin{equation}
%\norm{v-\hat{\mathbf{v}}}\leq \min\left\{\epsilon,\frac{8h\sqrt{n\ln(2)}}{\alpha\tau}\right\}\,.
%\end{equation}
%\end{proof}

